Co-occurring Associated REtained concepts in Diffusion Unlearning

Unlearning has emerged as a key technique to mitigate harmful content generation in diffusion models. However, existing methods often remove not only the target concept, but also benign co-occurring concepts. As illustrated in Fig.1, unlearning nudity can unintentionally suppress the concept of person, preventing a model from generating images with person. We define these undesirably suppressed co-occurring concepts that must be preserved CARE (Co-occurring Associated REtained concepts). Then, we introduce the CARE score, a general metric that directly quantifies their preservation across unlearning tasks. With this foundation, we propose ReCARE (Robust erasure for CARE), a framework that explicitly safeguards CARE while erasing only the target concept. ReCARE automatically constructs the CARE-set, a curated vocabulary of benign co-occurring tokens extracted from target images, and leverages this vocabulary during training for stable unlearning. Extensive experiments across various target concepts (Nudity, Van Gogh style, and Tench object) demonstrate that ReCARE achieves overall state-of-the-art performance in balancing robust concept erasure, overall utility, and CARE preservation.

==> table/care.tex <==

\begin{wraptable}{r}{0.38\textwidth} 
\vspace{-6.5mm}
\centering
\caption{Care.}
\label{care_clip}
\resizebox{0.38\textwidth}{!}{%
\begin{tabular}{@{}cccl@{}}
\toprule
\multirow{3}{*}{Model} & \multicolumn{3}{c}{\multirow{2}{*}{CARE score (↑)}}                            \\
                       & \multicolumn{3}{c}{}                                                     \\ \cmidrule(l){2-4} 
                       & Nudity               & vangogh              & \multicolumn{1}{c}{tench}  \\ \cmidrule(l){2-4} 
\textbf{SD v1.4}       & 0.2573               & 0.2634               & \multicolumn{1}{c}{0.2600} \\
\textbf{Ours}          & 0.2143               & 0.2583               & \multicolumn{1}{c}{0.2291} \\
\textbf{STEREO}        & 0.1754               & 0.2290               & \multicolumn{1}{c}{0.2004} \\
\textbf{ESD}           & 0.2206               & \multicolumn{1}{l}{} &                            \\
\textbf{AC}            & -                    & \multicolumn{1}{l}{} & \multicolumn{1}{c}{-}      \\
\textbf{UCE}           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                            \\
\textbf{AdvUnlearn}    & 0.1872               & 0.2435               & \multicolumn{1}{c}{0.1989} \\
\textbf{AGE}           & 0.2279               & 0.2598               & \multicolumn{1}{c}{0.2600} \\
\textbf{MACE}          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                            \\
\textbf{RECE}          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                            \\
\textbf{SPM}           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                            \\
\textbf{FMN}           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                            \\
\textbf{Salun}         & -                    & -                    &                            \\
\textbf{EraseDiff}     & -                    & -                    &                            \\ \bottomrule
\end{tabular}%
}
\end{wraptable}

==> table/care_exp.tex <==
\begin{table}[H]
\resizebox{\textwidth}{!}{%
% \caption{balance (Defense, Utility, CARE in Nudity Unlearning).}
\label{care_exp}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l
>{\columncolor[HTML]{FFFFFF}}c c
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c }
\hline
Metric  & \textbf{SD v1.4} & \textbf{FMN}                  & \textbf{SPM}                  & \textbf{ESD}                  & \textbf{UCE}                  & \textbf{AdvUnlearn}           & \textbf{AGE}                  & \textbf{MACE}                 & \textbf{RECE}                 & \textbf{STEREO} & {\color[HTML]{000000} \textbf{Ours}} \\ \hline
CARE    & 0.97             & 0.96                          & 0.95                          & 0.90                          & 0.95                          & \textbf{0.54}                 & \textbf{0.90}                 & -                             & 0.84                          & \textbf{0.40}   & {\color[HTML]{000000} \textbf{0.94}} \\
Defense & 43.18            & {\color[HTML]{000000} 48.18}  & {\color[HTML]{000000} 61.59}  & {\color[HTML]{000000} 46.59}  & {\color[HTML]{000000} 55.45}  & {\color[HTML]{000000} 34.55}  & {\color[HTML]{000000} 72.73}  & {\color[HTML]{000000} 38.18}  & {\color[HTML]{000000} 59.77}  & 80.45           & {\color[HTML]{000000} 88.86}         \\
Utility & 0.3136           & {\color[HTML]{000000} 0.3111} & {\color[HTML]{000000} 0.3125} & {\color[HTML]{000000} 0.3045} & {\color[HTML]{000000} 0.3117} & {\color[HTML]{000000} 0.3136} & {\color[HTML]{000000} 0.3006} & {\color[HTML]{000000} 0.2931} & {\color[HTML]{000000} 0.3097} & 0.2907          & {\color[HTML]{000000} 0.3053}       
\end{tabular}%
}
\end{table}

==> table/dictionary.tex <==
\begin{wraptable}{r}{0.3\textwidth} 
\begin{center}
\vspace{-5.0mm}
\captionof{table}{CARE score across different vocabularies on Ours}
\label{pre}
% \vspace{-1.0mm}
\resizebox{0.3\textwidth}{!}{%
\begin{tabular}{@{}ccc@{}}
              & \multicolumn{2}{c}{``A person''} \\ \cmidrule(l){2-3} 
dictionary        & Clip & CARE score \\ \midrule
ImageNet      &  -    & -           \\
Oxford-3K     &  -    & -           \\
GPT (co-occur) & -    & -            \\
Manual Anchor &  -   & -            \\
ours &  0.3053   & 0.95            \\
\end{tabular}%
}
\end{center}
% \vspace{-4.0mm}
\end{wraptable}

==> table/nudity_attack.tex <==
\begin{table}[]
\centering
\caption{Performance comparison on the \textit{Nudity} unlearning task.  
Evaluation is conducted under no attack (Erased) and three adversarial attacks (UD, RAB, CCE).  
We report \textbf{ASR} (robustness), \textbf{CLIP/FID} (utility on COCO-30K), and $\bm{\mathrm{CARE_\text{score}}}$ (CARE preservation).  
The overall performance is summarized by \textbf{RATIO}, our final aggregated metric that reflects the trade-off across all three dimensions. Full results with all baselines are provided in Appendix~\ref{full_result}.}
\label{nudity_attack}
\resizebox{0.78\textwidth}{!}{%
\begin{NiceTabular}{l||cccc|cc|c||c}
\CodeBefore
    \columncolor{lightgray}{1}
    \columncolor{lightgreen}{9}
\Body
\toprule
\midrule
 % -- 헤더 첫 번째 줄 --
 \multirow{2}{*}{\textbf{Method}} &
 \multicolumn{4}{c}{\textbf{Robustness}} &
 \multicolumn{2}{c}{\textbf{Utility}} &
 \textbf{CARE} &
 \multirow{2}{*}{\textbf{RATIO} $\uparrow$} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
 & \textbf{Erased} $\downarrow$ & \textbf{UD} $\downarrow$ & \textbf{RAB} $\downarrow$ & \textbf{CCE} $\downarrow$ &
   \textbf{CLIP} $\uparrow$ & \textbf{FID} $\downarrow$ & $\bm{\mathrm{CARE_\text{score}}}$ $\uparrow$ & \\
 \midrule
 % -- 표 본문 내용 --
 \textbf{SD v1.4}    & 35.23 & 39.51 & 56.52 & 56.82 & 0.3136 & 14.12 & 0.97 & 0.56 \\
 \textbf{ESD}        & 3.18  & 3.70  & 6.52  & 53.41 & 0.3045 & 13.75 & 0.89 & 0.49 \\
 \textbf{AdvUnlearn} & 23.64 & 1.23  & 0.00  & 65.45 & 0.2925 & 15.53 & 0.36 & 0.18 \\
 \textbf{AGE}        & 0.23  & 2.47  & 0.00  & 27.27 & 0.3006 & 11.25 & 0.79 & 0.56 \\
 \textbf{STEREO}     & 0.00  & 0.00  & 0.00  & 19.55 & 0.2907 & 17.83 & 0.11 & 0.21 \\
\midrule
 \textbf{Ours}       & 0.00  & 0.00  & 0.00  & 11.14 & 0.3053 & 13.85 & 0.94 & \textcolor{red}{0.76} \\
\midrule
\bottomrule
\end{NiceTabular}
}
\end{table}


==> table/nudity_attack_2.tex <==
\begin{table}[]
\centering
\caption{Performance comparison on the \textit{Nudity} unlearning task.  
Evaluation is conducted under no attack (Erased) and three adversarial attacks (UD, RAB, CCE).  
We report \textbf{ASR} (robustness), \textbf{CLIP/FID} (utility on COCO-30K), and $\bm{\mathrm{CARE_\text{score}}}$ (CARE preservation).  
The overall performance is summarized by \textbf{RATIO}, our final aggregated metric that reflects the trade-off across all three dimensions. Full results with all baselines are provided in Appendix~\ref{full_result}.}
\label{nudity_attack_2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c c
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
\multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}                              & \textbf{Metric}       & \textbf{SD v1.4} & \textbf{ESD} & \textbf{FMN} & \textbf{SPM} & \cellcolor[HTML]{FFFFFF}\textbf{AdvUnlearn} & \textbf{AGE} & \textbf{STEREO} & \textbf{Ours} \\ \hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{Erased ↓}     & 35.23            & 3.18         & 32.73        & 14.09        & \cellcolor[HTML]{FFFFFF}23.64               & 0.23         & 0.00            & 0.00          \\
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{UD ↓}         & 39.51            & 3.70         & 35.80        & 23.46        & \cellcolor[HTML]{FFFFFF}1.23                & 2.47         & 0.00            & 0.00          \\
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{RAB ↓}        & 56.52            & 6.52         & 60.87        & 9.78         & \cellcolor[HTML]{FFFFFF}0.00                & 0.00         & 0.00            & 0.00          \\
\multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}Robustness}} & \textbf{CCE ↓}        & 56.82            & 53.41        & 51.82        & 38.41        & \cellcolor[HTML]{FFFFFF}65.45               & 27.27        & 19.55           & 11.14         \\ \hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{CLIP ↑}       & 0.3136           & 0.3045       & 0.3111       & 0.3125       & 0.2925                                      & 0.3006       & 0.2907          & 0.3053        \\
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Utility}}    & \textbf{FID ↓}        & 14.12            & 13.75        & 13.95        & 14.62        & 15.53                                       & 11.25        & 17.83           & 13.85         \\ \hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}CARE}                         & \textbf{CARE score ↑} & 0.97             & 0.89         & 0.97         & 0.96         & \cellcolor[HTML]{FFFFFF}0.36                & 0.79         & 0.11            & 0.94          \\ \hline
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}ALL}                          & \textbf{Ratio  ↑}     & 0.5642           & 0.4901       & 0.5782       & 0.6661       & \cellcolor[HTML]{FFFFFF}0.1842              & 0.5571       & 0.2067          & 0.7580        \\ \hline
\end{tabular}
}
\end{table}


==> table/nudity_attack_3.tex <==
\begin{table}[]
\centering
\caption{Performance comparison on the \textit{Nudity} unlearning task.  
Evaluation is conducted under no attack (Erased) and three adversarial attacks (UD, RAB, CCE).  
We report \textbf{ASR} (robustness), \textbf{CLIP/FID} (utility on COCO-30K), and $\bm{\mathrm{CARE_\text{score}}}$ (CARE preservation).  
The overall performance is summarized by \textbf{RATIO}, our final aggregated metric that reflects the trade-off across all three dimensions. Full results with all baselines are provided in Appendix~\ref{full_result}.}
\label{vangogh_attack_3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\multicolumn{10}{}{nudity}                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}                              & \textbf{Metric}                         & \textbf{SD v1.4}               & \textbf{ESD}                   & \textbf{FMN}                   & \textbf{SPM}                   & \textbf{AdvUnlearn} & \textbf{AGE}                   & \textbf{STEREO}                & \textbf{Ours}                  \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{Erased ↓}                       & 35.23                          & 3.18                           & 32.73                          & 14.09                          & 23.64               & 0.23                           & 0.00                           & 0.00                           \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{UD ↓}                           & 39.51                          & 3.70                           & 35.80                          & 23.46                          & 1.23                & 2.47                           & 0.00                           & 0.00                           \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{RAB ↓}                          & 56.52                          & 6.52                           & 60.87                          & 9.78                           & 0.00                & 0.00                           & 0.00                           & 0.00                           \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}Robustness}} & \textbf{CCE ↓}                          & 56.82                          & 53.41                          & 51.82                          & 38.41                          & 65.45               & 27.27                          & 19.55                          & 11.14                          \\ \hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \cellcolor[HTML]{FFFFFF}\textbf{CLIP ↑} & \cellcolor[HTML]{FFFFFF}0.3136 & \cellcolor[HTML]{FFFFFF}0.3045 & \cellcolor[HTML]{FFFFFF}0.3111 & \cellcolor[HTML]{FFFFFF}0.3125 & 0.2925              & \cellcolor[HTML]{FFFFFF}0.3006 & \cellcolor[HTML]{FFFFFF}0.2907 & \cellcolor[HTML]{FFFFFF}0.3053 \\
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Utility}}    & \cellcolor[HTML]{FFFFFF}\textbf{FID ↓}  & \cellcolor[HTML]{FFFFFF}14.12  & \cellcolor[HTML]{FFFFFF}13.75  & \cellcolor[HTML]{FFFFFF}13.95  & \cellcolor[HTML]{FFFFFF}14.62  & 15.53               & \cellcolor[HTML]{FFFFFF}11.25  & \cellcolor[HTML]{FFFFFF}17.83  & \cellcolor[HTML]{FFFFFF}13.85  \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}CARE}                         & \textbf{CARE score ↑}                   & 0.97                           & 0.89                           & 0.97                           & 0.96                           & 0.36                & 0.79                           & 0.11                           & 0.94                           \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}ALL}                          & \textbf{Ratio  ↑}                       & 0.5642                         & 0.4901                         & 0.5782                         & 0.6661                         & 0.1842              & 0.5571                         & 0.2067                         & 0.7580                         \\ \hline
\multicolumn{10}{l}{vangogh}                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{Erased ↓}                       & 35.23                          & 3.18                           & 32.73                          & 14.09                          & 23.64               & 0.23                           & 0.00                           & 0.00                           \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{UD ↓}                           & \textbf{39.51}                 & 3.70                           & 35.80                          & 23.46                          & 1.23                & 2.47                           & 0.00                           & 0.00                           \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}Robustness}} & \textbf{CCE ↓}                          & \textbf{56.82}                 & 53.41                          & 51.82                          & 38.41                          & 65.45               & 27.27                          & 19.55                          & 11.14                          \\ \hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \cellcolor[HTML]{FFFFFF}\textbf{CLIP ↑} & \cellcolor[HTML]{FFFFFF}0.3136 & \cellcolor[HTML]{FFFFFF}0.3045 & \cellcolor[HTML]{FFFFFF}0.3111 & \cellcolor[HTML]{FFFFFF}0.3125 & 0.2925              & \cellcolor[HTML]{FFFFFF}0.3006 & \cellcolor[HTML]{FFFFFF}0.2907 & \cellcolor[HTML]{FFFFFF}0.3053 \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Utility}}    & \textbf{FID ↓}                          & \textbf{14.12}                 & 13.75                          & 13.95                          & 14.62                          & 15.53               & 11.25                          & 17.83                          & 13.85                          \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}CARE}                         & \textbf{CARE score ↑}                   & 0.97                           & 0.89                           & 0.97                           & 0.96                           & 0.36                & 0.79                           & 0.11                           & 0.94                           \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}ALL}                          & \textbf{Ratio  ↑}                       & 0.5642                         & 0.4901                         & 0.5782                         & 0.6661                         & 0.1842              & 0.5571                         & 0.2067                         & 0.7580                         \\ \hline
\multicolumn{10}{l}{tench}                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{Erased ↓}                       & 35.23                          & 3.18                           & 32.73                          & 14.09                          & 23.64               & 0.23                           & 0.00                           & 0.00                           \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \textbf{UD ↓}                           & \textbf{39.51}                 & \textbf{3.70}                  & 35.80                          & 23.46                          & 1.23                & 2.47                           & 0.00                           & 0.00                           \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}Robustness}} & \textbf{CCE ↓}                          & \textbf{56.82}                 & \textbf{53.41}                 & 51.82                          & 38.41                          & 65.45               & 27.27                          & 19.55                          & 11.14                          \\ \hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}}                             & \cellcolor[HTML]{FFFFFF}\textbf{CLIP ↑} & \cellcolor[HTML]{FFFFFF}0.3136 & \cellcolor[HTML]{FFFFFF}0.3045 & \cellcolor[HTML]{FFFFFF}0.3111 & \cellcolor[HTML]{FFFFFF}0.3125 & 0.2925              & \cellcolor[HTML]{FFFFFF}0.3006 & \cellcolor[HTML]{FFFFFF}0.2907 & \cellcolor[HTML]{FFFFFF}0.3053 \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Utility}}    & \textbf{FID ↓}                          & \textbf{14.12}                 & \textbf{13.75}                 & 13.95                          & 14.62                          & 15.53               & 11.25                          & 17.83                          & 13.85                          \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}CARE}                         & \textbf{CARE score ↑}                   & 0.97                           & 0.89                           & 0.97                           & 0.96                           & 0.36                & 0.79                           & 0.11                           & 0.94                           \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}ALL}                          & \textbf{Ratio  ↑}                       & 0.5642                         & 0.4901                         & 0.5782                         & 0.6661                         & 0.1842              & 0.5571                         & 0.2067                         & 0.7580                         \\ \hline
\end{tabular}
}
\end{table}


==> table/tench_attack.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison on the \textit{Tench} unlearning task.  
Evaluation is conducted under no attack (Erased) and two adversarial attacks (UD, CCE).  
We report \textbf{ASR} (robustness), \textbf{CLIP/FID} (utility on COCO-30K), and $\bm{\mathrm{CARE_\text{score}}}$ (CARE preservation).  
The overall performance is summarized by \textbf{RATIO}, our final aggregated metric that reflects the trade-off across all three dimensions. Full results with all baselines are provided in Appendix~\ref{full_result}.}
\label{tench_attack}
\resizebox{0.78\textwidth}{!}{%
\begin{NiceTabular}{l||ccc|cc|c||c}
\CodeBefore
    \columncolor{lightgray}{1}
    \columncolor{lightgreen}{8}
\Body
\midrule\midrule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c}{\textbf{Robustness}} &
\multicolumn{2}{c}{\textbf{Utility}} &
\textbf{CARE} &
\multirow{2}{*}{\textbf{RATIO ↑}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}
& \textbf{Erased ↓} & \textbf{UD ↓} & \textbf{CCE ↓} & 
  \textbf{CLIP ↑} & \textbf{FID ↓} & $\bm{\mathrm{CARE_\text{score}}}$ ↑ &  \\ \midrule
\textbf{SD v1.4}    & 96.80 & 92.00 & 98.00 & 0.3136 & 14.12 & 0.95 & 0.30 \\
\textbf{ESD}         & 3.80  & 40.00 & 94.80 & 0.3051 & 13.18 & 0.83 & 0.25 \\
\textbf{AdvUnlearn} & 0.00  & 2.00  & 95.20 & 0.3093 & 14.26 & 0.66 & 0.21 \\
\textbf{AGE}        & 63.80 & 96.00 & 99.40 & 0.3121 & 13.89 & 0.95 & 0.28 \\
\textbf{STEREO}     & 0.00  & 0.00  & 3.60  & 0.2975 & 15.87 & 0.62 & 0.56 \\ \midrule
\textbf{Ours}       & 0.00  & 0.00  & 0.40  & 0.3073 & 14.32 & 0.97 & \textcolor{red}{0.85} \\ 
\midrule\midrule
\end{NiceTabular}%
}
\vspace{-3.0mm}
\end{table}


==> table/tench_attack_ap.tex <==
\begin{table}[h]
\centering
\caption{Full performance comparison on the \textit{Tench} object unlearning task.}
\resizebox{0.9\textwidth}{!}{%
\begin{NiceTabular}{l||ccc|cc|c||c}
\CodeBefore
  \columncolor{lightgray}{1} % Method 열 회색
  \columncolor{lightgreen}{8} % Ratio 열 강조
\Body
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c}{\textbf{Robustness}} &
\multicolumn{2}{c}{\textbf{Utility}} &
\textbf{CARE} &
\multirow{2}{*}{\textbf{RATIO ↑}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}
& \textbf{Erased ↓} & \textbf{UD ↓} & \textbf{CCE ↓} & 
  \textbf{CLIP ↑} & \textbf{FID ↓} & $\bm{\mathrm{CARE_\text{score}}}$ ↑ &  \\ \midrule
\textbf{SD v1.4}     & 96.80 & 92.00 & 98.00 & 0.3136 & 14.12 & 0.95 & 0.30 \\
\textbf{ESD}         & 3.80  & 40.00 & 94.80 & 0.3051 & 13.18 & 0.83 & 0.25 \\
\textbf{FMN}         & 92.60 & 96.00 & 94.60 & 0.3114 & 13.42 & 0.95 & 0.31 \\
\textbf{SalUn}       & 0.00  & 2.00  & 91.60 & 0.3150 & 14.05 & 0.96 & 0.35 \\
\textbf{EraseDiff}   & 0.20  & 10.00 & 87.00 & 0.3120 & 12.62 & 0.93 & 0.35 \\
\textbf{SPM}         & 45.80 & 84.00 & 98.00 & 0.3134 & 14.05 & 0.96 & 0.30 \\
\textbf{AdvUnlearn}  & 0.00  & 2.00  & 95.20 & 0.3093 & 14.26 & 0.66 & 0.21 \\
\textbf{AGE}         & 63.80 & 96.00 & 99.40 & 0.3121 & 13.89 & 0.95 & 0.28 \\
\textbf{STEREO}      & 0.00  & 0.00  & 3.60  & 0.2975 & 15.87 & 0.62 & 0.56 \\ \midrule
\textbf{ReCARE (Ours)}        & 0.00  & 0.00  & 0.40  & 0.3073 & 14.32 & 0.97 & \textcolor{red}{0.85} \\ \bottomrule
\end{NiceTabular}%
}
\vspace{-3.0mm}
\end{table}


==> table/vangogh_attack.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison on the \textit{Van Gogh} style unlearning task.  
Evaluation is conducted under no attack (Erased) and two adversarial attacks (UD, CCE).  
We report \textbf{ASR} (robustness), \textbf{CLIP/FID} (utility on COCO-30K), and $\bm{\mathrm{CARE_\text{score}}}$ (CARE preservation).  
The overall performance is summarized by \textbf{Ratio}, our final aggregated metric that reflects the trade-off across all three dimensions. Full results with all baselines are provided in Appendix~\ref{full_result}.}
\label{vangogh_attack}
\resizebox{0.78\textwidth}{!}{%
\begin{NiceTabular}{l||ccc|cc|c||c}
\CodeBefore
    \columncolor{lightgray}{1}
    \columncolor{lightgreen}{8}
\Body
\midrule\midrule % <-- 제일 위선 이중선
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c}{\textbf{Robustness}} &
\multicolumn{2}{c}{\textbf{Utility}} &
\textbf{CARE} &
\multirow{2}{*}{\textbf{RATIO ↑}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}
& \textbf{Erased ↓} & \textbf{UD ↓} & \textbf{CCE ↓} & 
  \textbf{CLIP ↑} & \textbf{FID ↓} & $\bm{\mathrm{CARE_\text{score}}}$ ↑ &  \\ 
\midrule % <-- 헤더 아래 단일선
\textbf{SD v1.4}    & 74.00 & 84.00 & 64.40 & 0.3136 & 14.12 & 0.89 & 0.48 \\
\textbf{ESD}         & 0.40  & 18.00 & 13.20 & 0.3074 & 14.47 & 0.77 & 0.67 \\
\textbf{AdvUnlearn} & 0.80  & 4.00  & 57.00 & 0.3106 & 14.04 & 0.76 & 0.45 \\
\textbf{AGE}        & 0.00 & 14.00 & 12.40 & 0.3100 & 13.80 & 0.75 & 0.68 \\
\textbf{STEREO}     & 0.00  & 6.00  & 4.00  & 0.3047 & 18.17 & 0.31 & 0.43 \\ 
\midrule % <-- Ours 윗선도 이중선
\textbf{Ours}       & 0.00  & 6.00  & 6.00  & 0.3101 & 16.24 & 0.90 & \textcolor{red}{0.81} \\ 
\midrule\midrule % <-- 마지막도 이중선
\end{NiceTabular}%
}
\end{table}


==> table/vangogh_attack4.tex <==
\begin{table}[t]
\centering
\caption{Unified full comparison across \textit{Nudity}, \textit{Tench}, and \textit{Van Gogh} unlearning tasks. RAB is not evaluated for \textit{Tench} and \textit{Van Gogh} (marked as “—”).}
\label{tab:unified_all_nice}
\resizebox{0.98\textwidth}{!}{%
\begin{NiceTabular}{l|l||cccc|cc|c||c}
\CodeBefore
  \columncolor{lightgray}{1,2} % Task / Method
  \columncolor{lightgreen}{10} % RATIO
\Body
\toprule
\multicolumn{2}{c||}{} &
\multicolumn{4}{c|}{\textbf{Robustness (ASR ↓)}} &
\multicolumn{2}{c|}{\textbf{Utility}} &
\textbf{CARE} &
\textbf{RATIO ↑} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-8}\cmidrule(lr){9-9}
\multicolumn{2}{c||}{} & \textbf{Erased ↓} & \textbf{UD ↓} & \textbf{RAB ↓} & \textbf{CCE ↓} & \textbf{CLIP ↑} & \textbf{FID ↓} & $\bm{\mathrm{CARE_\text{score}}}$ \textbf{↑} &  \\
\midrule
\multirow{11}{*}{\textit{Nudity}} & \textbf{SD v1.4}    & 35.23 & 39.51 & 56.52 & 56.82 & 0.3136 & 14.12 & 0.97 & 0.56 \\
 & \textbf{ESD}        & 3.18  & 3.70  & 6.52  & 53.41 & 0.3045 & 13.75 & 0.89 & 0.49 \\
 & \textbf{FMN}        & 32.73 & 35.80 & 60.87 & 51.82 & 0.3111 & 13.95 & 0.95 & 0.31 \\
 & \textbf{UCE}        & 2.27  & 3.70  & 3.26  & 44.55 & 0.3117 & 14.31 & 0.83 & 0.48 \\
 & \textbf{SPM}        & 14.09 & 23.46 & 9.78  & 38.41 & 0.3125 & 14.62 & 0.96 & 0.30 \\
 & \textbf{MACE}       & 0.00  & 2.47  & 1.09  & 61.82 & 0.2931 & 12.70 & 0.95 & 0.10 \\
 & \textbf{RECE}       & 0.91  & 3.70  & 2.17  & 40.23 & 0.3097 & 14.62 & 0.83 & 0.51 \\
 & \textbf{AdvUnlearn} & 23.64 & 1.23  & 0.00  & 65.45 & 0.2925 & 15.53 & 0.36 & 0.18 \\
 & \textbf{AGE}        & 0.23  & 2.47  & 0.00  & 27.27 & 0.3006 & 11.25 & 0.79 & 0.56 \\
 & \textbf{STEREO}     & 0.00  & 0.00  & 0.00  & 19.55 & 0.2907 & 17.83 & 0.11 & 0.21 \\
 & \textbf{Ours}       & 0.00  & 0.00  & 0.00  & 11.14 & 0.3053 & 13.85 & 0.94 & \textcolor{red}{0.7580} \\
\midrule
\multirow{12}{*}{\textit{Tench}} & \textbf{SD v1.4}     & 74.00 & 84.00 & —    & 64.40 & 0.3136 & 14.12 & 0.89 & 0.48 \\
 & \textbf{ESD}         & 0.40  & 18.00 & —    & 13.20 & 0.3074 & 14.47 & 0.77 & 0.67 \\
 & \textbf{FMN}         & 1.60  & 14.00 & —    & 61.60 & 0.3140 & 13.90 & 0.85 & 0.48 \\
 & \textbf{AC}          & 2.40  & 48.00 & —    & 36.00 & 0.3124 & 14.04 & 0.90 & 0.65 \\
 & \textbf{UCE}         & 20.60 & 76.00 & —    & 61.80 & 0.3140 & 13.88 & 0.84 & 0.48 \\
 & \textbf{SPM}         & 9.60  & 60.00 & —    & 54.60 & 0.3134 & 14.06 & 0.82 & 0.51 \\
 & \textbf{MACE}        & 5.60  & 20.00 & —    & 52.40 & 0.2862 & 12.60 & 0.05 & 0.10 \\
 & \textbf{RECE}        & 2.40  & 42.00 & —    & 55.80 & 0.3137 & 13.84 & 0.83 & 0.51 \\
 & \textbf{AdvUnlearn}  & 0.80  & 4.00  & —    & 57.00 & 0.3106 & 14.04 & 0.76 & 0.4523 \\
 & \textbf{AGE}         & 0.00  & 14.00 & —    & 12.40 & 0.3100 & 13.80 & 0.75 & 0.68 \\
 & \textbf{STEREO}      & 0.00  & 6.00  & —    & 4.00  & 0.3047 & 18.17 & 0.31 & 0.43 \\
 & \textbf{Ours}        & 0.00  & 6.00  & —    & 6.00  & 0.3101 & 16.24 & 0.90 & \textcolor{red}{0.81} \\
\midrule
\multirow{10}{*}{\textit{Van Gogh}} & \textbf{SD v1.4}     & 96.80 & 92.00 & —    & 98.00 & 0.3136 & 14.12 & 0.95 & 0.30 \\
 & \textbf{ESD}         & 3.80  & 40.00 & —    & 94.80 & 0.3051 & 13.18 & 0.83 & 0.25 \\
 & \textbf{FMN}         & 92.60 & 96.00 & —    & 94.60 & 0.3114 & 13.42 & 0.95 & 0.31 \\
 & \textbf{SalUn}       & 0.00  & 2.00  & —    & 91.60 & 0.3150 & 14.05 & 0.96 & 0.35 \\
 & \textbf{EraseDiff}   & 0.20  & 10.00 & —    & 87.00 & 0.3120 & 12.62 & 0.93 & 0.35 \\
 & \textbf{SPM}         & 45.80 & 84.00 & —    & 98.00 & 0.3134 & 14.05 & 0.96 & 0.30 \\
 & \textbf{AdvUnlearn}  & 0.00  & 2.00  & —    & 95.20 & 0.3093 & 14.26 & 0.66 & 0.21 \\
 & \textbf{AGE}         & 63.80 & 96.00 & —    & 99.40 & 0.3121 & 13.89 & 0.95 & 0.28 \\
 & \textbf{STEREO}      & 0.00  & 0.00  & —    & 3.60  & 0.2975 & 15.87 & 0.62 & 0.56 \\
 & \textbf{Ours}        & 0.00  & 0.00  & —    & 0.40  & 0.3073 & 14.32 & 0.97 & \textcolor{red}{0.85} \\
\bottomrule
\end{NiceTabular}%
}
\end{table}


==> table/vangogh_attack_ap.tex <==
\begin{table}[H]
\centering
\caption{Full performance comparison on the \textit{Van Gogh} style unlearning task.}
\resizebox{0.9\textwidth}{!}{%
\begin{NiceTabular}{l||ccc|cc|c||c}
\CodeBefore
  \columncolor{lightgray}{1} % Method 열 회색
  \columncolor{lightgreen}{8} % Ratio 열 강조
\Body
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c}{\textbf{Robustness}} &
\multicolumn{2}{c}{\textbf{Utility}} &
\textbf{CARE} &
\multirow{2}{*}{\textbf{RATIO ↑}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}
& \textbf{Erased ↓} & \textbf{UD ↓} & \textbf{CCE ↓} & 
  \textbf{CLIP ↑} & \textbf{FID ↓} & $\bm{\mathrm{CARE_\text{score}}}$ ↑ &  \\ \midrule
\textbf{SD v1.4}     & 74.00 & 84.00 & 64.40 & 0.3136 & 14.12 & 0.89 & 0.48 \\
\textbf{ESD}         & 0.40  & 18.00 & 13.20 & 0.3074 & 14.47 & 0.77 & 0.67 \\
\textbf{FMN}         & 1.60  & 14.00 & 61.60 & 0.3140 & 13.90 & 0.85 & 0.48 \\
\textbf{AC}          & 2.40  & 48.00 & 36.00 & 0.3124 & 14.04 & 0.90 & 0.65 \\
\textbf{UCE}         & 20.60 & 76.00 & 61.80 & 0.3140 & 13.88 & 0.84 & 0.48 \\
\textbf{SPM}         & 9.60  & 60.00 & 54.60 & 0.3134 & 14.06 & 0.82 & 0.51 \\
\textbf{MACE}        & 5.60  & 20.00 & 52.40 & 0.2862 & 12.60 & 0.05 & 0.10 \\
\textbf{RECE}        & 2.40  & 42.00 & 55.80 & 0.3137 & 13.84 & 0.83 & 0.51 \\
\textbf{AdvUnlearn} & 0.80  & 4.00  & 57.00 & 0.3106  & 14.04   & 0.76 & 0.45 \\
\textbf{AGE}         & 0.00  & 14.00 & 12.40 & 0.3100 & 13.80 & 0.75 & 0.68 \\
\textbf{STEREO}      & 0.00  & 6.00  & 4.00  & 0.3047 & 18.17 & 0.31 & 0.43 \\ \midrule
\textbf{ReCARE (Ours)}        & 0.00  & 6.00  & 6.00  & 0.3101 & 16.24 & 0.90 & \textcolor{red}{0.81} \\ \bottomrule
\end{NiceTabular}%
}
\end{table}


==> table/yes_ratio.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.35\linewidth}{!}{
    \begin{tabular}{lc}
        \toprule
        \textbf{Target} & \textbf{Validity Rate (YES Ratio)} \\
        \midrule
        Nudity   & 0.914 \\
        Van Gogh & 0.909 \\
        Tench    & 0.949 \\
        \bottomrule
    \end{tabular}}
    \caption{\textcolor{magenta}{LLM-based semantic validation results of automatically extracted CARE-sets.}}
    \label{tab:yes_ratio}
\end{table}
